Revisiting Model Stitching to Compare Neural Representations

We revisit and extend model stitching (Lenc & Vedaldi 2015) as a methodology to study the internal representations of neural networks. Given two trained and frozen models $A$ and $B$, we consider a "stitched model'' formed by connecting the bottom-layers of $A$ to the top-layers of $B$, with a simple trainable layer between them. We argue that model stitching is a powerful and perhaps under-appreciated tool, which reveals aspects of representations that measures such as centered kernel alignment (CKA) cannot. Through extensive experiments, we use model stitching to obtain quantitative verifications for intuitive statements such as "good networks learn similar representations'', by demonstrating that good networks of the same architecture, but trained in very different ways (e.g.: supervised vs. self-supervised learning), can be stitched to each other without drop in performance. We also give evidence for the intuition that "more is better'' by showing that representations learnt with (1) more data, (2) bigger width, or (3) more training time can be "plugged in'' to weaker models to improve performance. Finally, our experiments reveal a new structural property of SGD which we call "stitching connectivity'', akin to mode-connectivity: typical minima reached by SGD can all be stitched to each other with minimal change in accuracy.

==> checklist.tex <==

\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}{}
  \item Did you describe the limitations of your work?
    \answerYes{In Section \ref{sec:conclude}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{ In Section \ref{sec:conclude}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The code is based on standard CIFAR-10 ImageNet training and we provide sufficient details in \ref{app:exp-details} to reproduce the experiments}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Experimental details are discussed in Appendix \ref{app:exp-details}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Due to the expensive computational nature of these experiments, we do not report errors bars. This is standard practice in such work, and we do not expect variability in the qualtitative results to change as has been shown before in CIFAR-10 and ImageNet training}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, Appendix \ref{app:exp-details}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> old_experiments.tex <==
\section{Experiments}
\pnote{old section... merge into the above}

\subsection{Setup}
Unless specified otherwise, the CIFAR-10 experiments are conducted on the ResNet-20 architecture from \citet{he2015deep} with a width multiplier of $4\times$. For the ImageNet experiments, we use the ResNet-50 architecture \cite{he2015deep}. The ResNets are trained with the standard hyperparameters. The stitching layer in the ResNets consists of a $1\times1$ convolutional layer. We add a BatchNorm (BN) layer before and after this convolutional layer. Note that the BN layer does not change the representation capacity of the stitching layer and only aides with optimization. We perform stitching only between ResNet blocks (and not inside a block), but note that it is possible to stitch within the block as well. We use the Adam optimizer with the cosine learning rate decay and an initial learning rate of $0.001$. Full experimental details are described in Appendix \ref{?}.

\subsection{Sanity Checks}

{\bf Random networks:} One possible failure mode of stitching can occur when the family of stitchers $\cS$ is powerful enough to learn to map any two arbitrary representations onto each other. To avoid this, we use a very simple linear $1\times1$ convolutional stitching layer. To verify that our experiments are not in such a regime, we stitch a randomly initialized network with a fully trained network. Figure \ref{?} shows that the penalty of such a stitched network increases quickly with stitching depth. 

{\bf Comparison with CKA:} We repeat the experiment conducted by \cite{Kornblith0LH19} to identify which layer a representation came from when comparing two networks of two random initializations. We find that the similar layers are similar to each other as shown in Figure \ref{}. Note that in some cases, the layer 1 or 2 above the comparison layer may have lower penalty than the exact layer. TODO: Discuss this - maybe we want to define similarity as $P(i, j) + P(j, i) / 2$ to make it symmetric?
\pnote{actually we're not including this exp anymore right?}


